Modeling Intensification for Sign Language Generation: A Computational Approach

End-to-end sign language generation models do not accurately represent the prosody in sign language. A lack of temporal and spatial variations leads to poor-quality generated presentations that confuse human interpreters. In this paper, we aim to improve the prosody in generated sign languages by modeling intensification in a data-driven manner. We present different strategies grounded in linguistics of sign language that inform how intensity modifiers can be represented in gloss annotations. To employ our strategies, we first annotate a subset of the benchmark PHOENIX-14T, a German Sign Language dataset, with different levels of intensification. We then use a supervised intensity tagger to extend the annotated dataset and obtain labels for the remaining portion of it. This enhanced dataset is then used to train state-of-the-art transformer models for sign language generation. We find that our efforts in intensification modeling yield better results when evaluated with automatic metrics. Human evaluation also indicates a higher preference of the videos generated using our model.

==> todo.tex <==
% x make the human annotation table a pie chart - S (done)
% - put some examples from the human annotation skeletons for the evaluation M
% - visual representation of the heuristics 
% x write the conclusion - M
% x write the abstract
% - check for consistency over the abbreviations, usage of terminology overall - S
% x change w/label w/o label - Y (done)
% - write the ethics section (check malihe's prev papers for ref) - S
% - put the model diagram M
% x compress the table in the first figure -Y (done)
% - remove non-scientific jargon 
% x add the bleu-1-2-3 scores with their significance in another table maybe - Y (done)
% x extend introduction with related work
% - include more of the main argument of the paper! it should be connected in each section (connected back) (we are the first one to do data-driven way) (focus on how our work is different, although there has been work)
% - generation not production!
% x combine table 3 and 4 and maybe flip the table?
% - change the human eval figure (more professional)
% - mention the explanation for the difference between B4 in w/intensity and w/o intensity in the analysis section
% - make the figure/table captions with the takeaway message

% ## NEW TODO after Nov 11 meeting
% x Add words on the release of dataset and code - Y (done)
% x Revise the Introduction, start with the core story: study modifiers in sign language -- already work in linguistics with citations, pointed out interesting, but unexplored area in sign lanuage. - M 
% x In introduction, instead of stating the findings, start with "we hypothesized xxx" - M 
% x Remove Background and add the contents to Introduction and later added "Heuristics for Intensification" section - M and Y 
% x Remove Data and merge into "Heuristics" section, refer to Malihe's CLUE paper. - Y  Y (done)
% x Introduce the sign gloss - Y 
% x Improve Figure 2 caption - M 
% x revise the model details - Y  Y (done)
% - Finish the analyis, ideally with human evaluations and real examples to demonstrate the quality. - S 
% - Remove Accuracy/P/R from Table 2 and run significance test. - S
% - Cite the Vlogging paper - M

-Title: Singed —> sign X 
Abstract: 
-first sentence: "the languages"? doesn’t make sense. You need to revise this senesce X
-Second sentence: what does THIS refer to? Maybe you would want to use THE? Poor quality in what? What does lower human perception mean? X

-We seek to improve —> this sentence is too long. Improve in what sense? maybe it’s best to just talk about intensification here. X

-What strategies?  X

-We don’t extend the tagging, we extend the annotated dataset. X

-Regarding human evolution, significant performance is ambiguous. What do you mean by performance here? be more specific. X

-Mention the language that you are working with e.g. German sign language. you need to mention later in the discussion and conclusion what you chose to work with this dataset because we don't have ... X

Introduction 
-Plan an important role —> plan important roles X
-Maybe elaborate here by saying why it is important. Instead of AND between singed and spoken maybe you can use similar to spoken languages X
-Generation systems do not model prosody, they need to learn properly from data and generate presentations that respect prosody or generate presentations with better prosody X
-"HOWEVER", what is the contrast? Why are these two sentences contacted with HOWEVER? X
-From “however” until the end of the paragraph, I don’t understand what you are trying to say? the message is not clear. It’s all over the place. X
-take out "Evidently” and “potential” X
-Mapping—> mappings X
-Of state of the art models —> of the state of the art models X
-Prosody does not change with semantics. This needs an example. It’s not clear what you are referring to ...
-Add a link to a well-organized github repo with code and data to the intro. X
